IPBoost -- Non-Convex Boosting via Integer Programming

Recently non-convex optimization approaches for solving machine learning problems have gained significant attention. In this paper we explore non-convex boosting in classification by means of integer programming and demonstrate real-world practicability of the approach while circumventing shortcomings of convex boosting approaches. We report results that are comparable to or better than the current state-of-the-art.

==> tables/table-libsvm-overview.tex <==
% generated by paper_generate_overview_table.sh
\begin{table*}[t]
   \small
   \caption{Aggregated results for LIBSVM: Average test/train accuracies and standard deviations (STD) for three algorithms over 
            10 different seeds, using class probabilities for prediction and voting; we considered 40 instances 
            as outlined in Section~\ref{sec:comp-results}. Column ``\#~best'' represents the number of instances 
            on which the corresponding algorithm performed best (ties possible). Column ``ER'' gives the error rate,
            i.e., \(1/(1-a)\) for the average accuracy~\(a\).}
   \label{tab:aggregated}
   \begin{tabular*}{\textwidth}{@{}l@{\quad\extracolsep{\fill}}rrrrrrrrrrrrr@{}}\toprule
      && \multicolumn{4}{c}{IPBoost} & \multicolumn{4}{c}{LPBoost} & \multicolumn{4}{c}{AdaBoost}\\
         \cmidrule(lr){3-6}\cmidrule(lr){7-10}\cmidrule(l){11-14}
      type & \(\rho\)   & \# best & accuracy & STD & ER & \# best & accuracy & STD & ER & \# best & accuracy & STD & ER \\
      \midrule
 test & \num{  0.1} & \num{24} & \num{80.70} & \num{ 4.08} & \num{ 5.18} & \num{ 7} & \num{80.16} & \num{ 3.93} & \num{ 5.04} & \num{ 9} & \num{79.79} & \num{ 3.82} & \num{ 4.95}\\
 test & \num{0.075} & \num{25} & \num{80.77} & \num{ 3.89} & \num{ 5.20} & \num{ 6} & \num{80.21} & \num{ 3.89} & \num{ 5.05} & \num{ 9} & \num{79.79} & \num{ 3.82} & \num{ 4.95}\\
 test & \num{ 0.05} & \num{26} & \num{80.78} & \num{ 4.07} & \num{ 5.20} & \num{ 7} & \num{80.31} & \num{ 3.73} & \num{ 5.08} & \num{ 8} & \num{79.79} & \num{ 3.82} & \num{ 4.95}\\
 test & \num{0.025} & \num{25} & \num{80.63} & \num{ 3.94} & \num{ 5.16} & \num{ 7} & \num{80.21} & \num{ 3.91} & \num{ 5.05} & \num{ 8} & \num{79.79} & \num{ 3.82} & \num{ 4.95}\\
 test & \num{ 0.01} & \num{26} & \num{80.59} & \num{ 3.91} & \num{ 5.15} & \num{ 7} & \num{79.80} & \num{ 3.67} & \num{ 4.95} & \num{ 7} & \num{79.79} & \num{ 3.82} & \num{ 4.95}\\
      \midrule
train & \num{  0.1} & \num{25} & \num{83.52} & \num{ 2.51} & \num{ 6.07} & \num{ 1} & \num{82.29} & \num{ 2.61} & \num{ 5.65} & \num{15} & \num{84.36} & \num{ 1.99} & \num{ 6.40}\\
train & \num{0.075} & \num{24} & \num{83.94} & \num{ 2.38} & \num{ 6.23} & \num{ 1} & \num{82.52} & \num{ 2.54} & \num{ 5.72} & \num{15} & \num{84.36} & \num{ 1.99} & \num{ 6.40}\\
train & \num{ 0.05} & \num{26} & \num{84.34} & \num{ 2.43} & \num{ 6.38} & \num{ 1} & \num{82.90} & \num{ 2.40} & \num{ 5.85} & \num{14} & \num{84.36} & \num{ 1.99} & \num{ 6.40}\\
train & \num{0.025} & \num{29} & \num{84.97} & \num{ 2.44} & \num{ 6.65} & \num{ 1} & \num{83.39} & \num{ 2.43} & \num{ 6.02} & \num{10} & \num{84.36} & \num{ 1.99} & \num{ 6.40}\\
train & \num{ 0.01} & \num{31} & \num{85.69} & \num{ 2.48} & \num{ 6.99} & \num{ 3} & \num{84.20} & \num{ 2.26} & \num{ 6.33} & \num{ 6} & \num{84.36} & \num{ 1.99} & \num{ 6.40}\\
      \bottomrule
   \end{tabular*}
\end{table*}


==> tables/table-libsvm-runtimes.tex <==
% generated by paper_generate_pred_tables.sh
\begin{table}
   \small
   \caption{Statistics for LIBSVM on average run times (in seconds) of different algorithms with $\rho = 0.05$ for 10 different seeds;
            ``\#~optimal'' gives the number of instances solved to optimality, ``\#~time out'' the number of instances that ran into the
            time limit of 1 hour, and ``best sol.\ time'' the average time at which the best solution was found.}
   \label{tab:runtimeStats}
   \begin{tabular*}{\textwidth}{@{}l@{\extracolsep{\fill}}rrrrrrr@{}}\toprule
      & \multicolumn{4}{c}{IPBoost} & &  \\ \cmidrule(r){2-6}
      name & total time & \# nodes & \# optimal & \# time out & best sol.\ time & LPBoost time & AdaBoost time \\ \midrule
                      a1a & \num{  97.26} & \num{ 6669.9} &  0 &  0 & \num{  26.08} & \num{   0.15} & \num{   0.40} \\
                      a2a & \num{ 257.97} & \num{ 8186.6} &  0 &  0 & \num{ 128.55} & \num{   0.26} & \num{   0.59} \\
                      a3a & \num{ 464.05} & \num{ 9096.6} &  0 &  0 & \num{ 230.18} & \num{   0.37} & \num{   0.59} \\
                      a4a & \num{ 770.89} & \num{ 9769.9} &  0 &  0 & \num{ 381.76} & \num{   0.73} & \num{   0.83} \\
                      a5a & \num{ 904.72} & \num{10186.5} &  0 &  0 & \num{ 465.58} & \num{   1.11} & \num{   1.16} \\
                      a6a & \num{1712.09} & \num{ 7763.4} &  0 &  1 & \num{ 736.32} & \num{   2.76} & \num{   1.76} \\
                      a7a & \num{2946.71} & \num{ 8986.1} &  0 &  3 & \num{1542.57} & \num{   5.40} & \num{   2.74} \\
                      a8a & \num{3251.73} & \num{ 6370.4} &  0 &  8 & \num{2217.36} & \num{   9.33} & \num{   3.51} \\
                      a9a & \num{3247.98} & \num{ 4094.4} &  0 &  7 & \num{1461.27} & \num{  17.96} & \num{   4.89} \\
        australian\_scale & \num{  66.84} & \num{ 7400.4} &  1 &  0 & \num{  23.78} & \num{   0.07} & \num{   0.17} \\
     breast-cancer\_scale & \num{ 435.32} & \num{ 7183.9} &  0 &  1 & \num{  29.21} & \num{   0.06} & \num{   0.15} \\
                  cod-rna & \num{3603.83} & \num{   77.4} &  0 & 10 & \num{ 304.28} & \num{3281.72} & \num{  30.13} \\
             colon-cancer & \num{   0.09} & \num{    6.8} & 10 &  0 & \num{   0.02} & \num{   0.04} & \num{   0.21} \\
                     duke & \num{   0.25} & \num{    7.9} & 10 &  0 & \num{   0.03} & \num{   0.14} & \num{   0.37} \\
             german.numer & \num{  78.61} & \num{ 7215.8} &  0 &  0 & \num{  19.77} & \num{   0.09} & \num{   0.20} \\
           gisette\_scale & \num{3439.67} & \num{ 3709.8} &  0 &  8 & \num{1991.59} & \num{  18.87} & \num{  16.31} \\
          diabetes\_scale & \num{ 116.58} & \num{ 7313.7} &  0 &  0 & \num{  47.29} & \num{   0.07} & \num{   0.17} \\
         fourclass\_scale & \num{ 165.46} & \num{ 9932.6} &  0 &  0 & \num{ 102.16} & \num{   0.07} & \num{   0.16} \\
      german.numer\_scale & \num{ 120.73} & \num{ 9495.2} &  0 &  0 & \num{  62.95} & \num{   0.09} & \num{   0.20} \\
             heart\_scale & \num{  43.55} & \num{10170.0} &  0 &  0 & \num{  21.58} & \num{   0.03} & \num{   0.14} \\
                   ijcnn1 & \num{3604.29} & \num{ 1197.2} &  0 & 10 & \num{ 708.19} & \num{ 206.01} & \num{   5.95} \\
        ionosphere\_scale & \num{  67.56} & \num{ 7375.7} &  0 &  0 & \num{  24.33} & \num{   0.08} & \num{   0.16} \\
                      leu & \num{   0.20} & \num{    5.8} & 10 &  0 & \num{   0.02} & \num{   0.11} & \num{   0.34} \\
          liver-disorders & \num{  48.69} & \num{ 9768.9} &  0 &  0 & \num{  24.51} & \num{   0.04} & \num{   0.14} \\
                  madelon & \num{2387.03} & \num{ 7619.7} &  0 &  5 & \num{1354.16} & \num{   1.59} & \num{   0.90} \\
                mushrooms & \num{ 968.38} & \num{ 6761.5} &  0 &  0 & \num{ 248.43} & \num{   2.45} & \num{   1.42} \\
                 phishing & \num{ 977.76} & \num{ 6726.0} &  0 &  0 & \num{ 268.98} & \num{   3.76} & \num{   1.03} \\
            skin\_nonskin & \num{3576.38} & \num{ 2251.6} &  0 &  8 & \num{ 861.25} & \num{2967.50} & \num{   9.39} \\
             sonar\_scale & \num{  61.81} & \num{ 6531.4} &  0 &  0 & \num{  19.13} & \num{   0.07} & \num{   0.15} \\
                   splice & \num{ 128.63} & \num{ 5767.6} &  0 &  0 & \num{  25.33} & \num{   0.32} & \num{   0.28} \\
                svmguide1 & \num{1375.33} & \num{ 9187.1} &  0 &  0 & \num{ 685.39} & \num{   0.97} & \num{   0.39} \\
                svmguide3 & \num{ 671.57} & \num{10522.1} &  0 &  0 & \num{ 400.04} & \num{   0.38} & \num{   0.22} \\
                      w1a & \num{ 673.90} & \num{ 8291.2} &  0 &  0 & \num{ 240.40} & \num{   3.28} & \num{   6.05} \\
                      w2a & \num{ 927.73} & \num{ 7860.0} &  0 &  0 & \num{ 353.33} & \num{   3.53} & \num{   6.23} \\
                      w3a & \num{1665.23} & \num{ 8071.0} &  0 &  0 & \num{ 601.93} & \num{   3.80} & \num{   6.30} \\
                      w4a & \num{2442.22} & \num{ 8113.1} &  0 &  3 & \num{1256.18} & \num{   3.97} & \num{   6.36} \\
                      w5a & \num{2583.16} & \num{ 8091.4} &  0 &  2 & \num{1027.12} & \num{   4.53} & \num{   6.55} \\
                      w6a & \num{3607.69} & \num{ 5791.5} &  0 & 10 & \num{1881.83} & \num{   6.17} & \num{   7.42} \\
                      w7a & \num{3607.88} & \num{ 4362.3} &  0 & 10 & \num{2106.27} & \num{   7.79} & \num{   7.97} \\
                      w8a & \num{3611.46} & \num{ 3204.5} &  0 & 10 & \num{2022.04} & \num{  18.14} & \num{  11.50} \\
\midrule

                 averages & \num{1367.78} & \num{ 6528.4} & \num{0.8} & \num{2.4} & \num{ 597.53} & \num{ 164.35} & \num{   3.59} \\
      \bottomrule
   \end{tabular*}
\end{table}

